Reliabuild: Searching for High-Fidelity Builds Using Active Learning

Modern software is incredibly complex. A typical application may comprise hundreds or thousands of reusable components. Automated package managers can help to maintain a consistent set of dependency versions, but ultimately the solvers in these systems rely on constraints generated by humans. At scale, small errors add up, and it becomes increasingly difficult to find high-fidelity configurations. We cannot test all configurations, because the space is combinatorial, so exhaustive exploration is infeasible. In this paper, we present Reliabuild, an auto-tuning framework that efficiently explores the build configuration space and learns which package versions are likely to result in a successful configuration. We implement two models in Reliabuild to rank the different configurations and use adaptive sampling to select good configurations with fewer samples. We demonstrate Reliabuild's effectiveness by evaluating 31,186 build configurations of 61 packages from the Extreme-scale Scientific Software Stack(E4S). Reliabuild selects good configurations efficiently. For example, Reliabuild selects 3X the number of good configurations in comparison to random sampling for several packages including Abyss, Bolt, libnrm, OpenMPI. Our framework is also able to select all the high-fidelity builds in half the number of samples required by random sampling for packages such as Chai, OpenMPI, py-petsc4py, and slepc. We further use the model to learn statistics about the compatibility of different packages, which will enable package solvers to better select high-fidelity build configurations automatically.

==> config-selection.tex <==
\section{Configuration Selection}

We represent $i$th package by a random variable $X_i$ and values it can take by $x_i \in \{v_{i,1},\dots, v_{i,m_i}\}$.
We aim to select a valid configuration $x \equiv \{x_1,\dots,x_n\} \in \mathcal X$  
from the space of all possible configurations $\mathcal{X}$. 

In our context, each dimension 
of this space is categorical $V_i={v_{i,1},\dots, v_{i,m_i}}$, and is used to indicate the version or the
variant available for that package. Associated with $X$ is a DAG, $\mathcal{D}$,
depicting the dependency structure of the packages. We assume that each input dimension 
is only active under some instantiation of its  ancestor dimensions in $\mathcal{D}$. 
Moreover, the categorical values for each dimension are also affected by the ancestor 
instantiations. We define function $\delta_i: X \longrightarrow \hat{V}$, for $i\in{1,\dots,D}$ 
and $\hat{V}\subseteq V_i$. For a configuration $\hat{x}$, currently being constructed

$\delta_i(\hat{x}) = \delta_i(\hat{x}(anc_i))$

where $anc_i$ are the ancestors of $i$ in $\mathcal{D}$, such that the values available
for vertex $i$ are those that satisfy criteria based on the values for the $anc_i$ in $\hat{x}$.
If $\hat{V}_i = \emptyset$, then vertex $i$ is not active.

We use \emph{Sequential Model Based Optimization (SMBO)} for our configuration selection
problem. It iterates between fitting models and using them to make choices about which
configurations to investigate. 
The kernel function for modeling the objective function needs to account for the parameters
that are relevant as well as their values. 



==> intro-1.tex <==
\section{Introduction}
While package managers can automate the process of building and installing a software, they  depend on users to provide valid configurations. Selecting a configuration is typically done manually through trial and error, and requires in-depth understanding of package dependencies and their compatibility. For a decent sized software, this dependency graph can easily contain hundreds of packages each with several choices for version and variants. Exhaustive exploring of this large combinatorial configuration space is infeasible and user specified configuration might not necessarily be the most optimal one. Therefore, we need to apply autotuning methods to find valid and high quality configurations. 
 
We are developing an active learning based method to select valid configurations.  Our approach starts off by representing the relationship between a package and its dependencies as a graph, where an edge indicates a dependency and contains attributes for constraint rules. To bootstrap our learning algorithm, we require a random set of configurations that uniformly span the configuration space. 
To generate this random set of configurations, we use Metropolis Hastings algorithm on the dependency package graph choosing the versions and variants of all the relevant packages in the graph. 
The choice of version and variant for a package  can constrain the set of versions for its dependencies which are given by the constraint rules. 
Therefore, we select the parent’s version before exploring the children (which are the dependencies). Once we have assigned a version and a variant for all the valid packages, we have created a valid configuration. This initial set of random configurations are used as training samples for our active learning based model. 
In the next step, we plan to build a model based on Bayesian optimization method, where we will use the initial set of valid and invalid configurations to construct probability densities for package version and variant choices and draw samples from this distribution. We will use this as a guide for our ASP constraint solver to find and guarantee a valid configuration.


We look at a specific scenario where given a package with no prior information about valid configurations, we want to identify configurations that are highly likely to concretize and build. 
 

==> method.tex <==
\section{Configuration Selection}

We represent $i$th package by a random variable $X_i$ and values it can take by $x_i \in \{v_{i,1},\dots, v_{i,m_i}\}$.
We aim to select a valid configuration $x \equiv \{x_1,\dots,x_n\} \in \mathcal X$  
from the space of all possible configurations $\mathcal{X}$. 

In our context, each dimension 
of this space is categorical $V_i={v_{i,1},\dots, v_{i,m_i}}$, and is used to indicate the version or the
variant available for that package. Associated with $X$ is a DAG, $\mathcal{D}$,
depicting the dependency structure of the packages. We assume that each input dimension 
is only active under some instantiation of its  ancestor dimensions in $\mathcal{D}$. 
Moreover, the categorical values for each dimension are also affected by the ancestor 
instantiations. We define function $\delta_i: X \longrightarrow \hat{V}$, for $i\in{1,\dots,D}$ 
and $\hat{V}\subseteq V_i$. For a configuration $\hat{x}$, currently being constructed

$\delta_i(\hat{x}) = \delta_i(\hat{x}(anc_i))$

where $anc_i$ are the ancestors of $i$ in $\mathcal{D}$, such that the values available
for vertex $i$ are those that satisfy criteria based on the values for the $anc_i$ in $\hat{x}$.
If $\hat{V}_i = \emptyset$, then vertex $i$ is not active.

We use \emph{Sequential Model Based Optimization (SMBO)} for our configuration selection
problem. It iterates between fitting models and using them to make choices about which
configurations to investigate. 
The kernel function for modeling the objective function needs to account for the parameters
that are relevant as well as their values. 



==> mh-algo.tex <==
\subsection{Random sampling using Metropolis Hastings algorithm}

Random walk Metropolis algorithm is a first order Markov Chain Monte Carlo
algorithm. It is a type of dependent sampling algorithm because where we
sample next is dependent on where we are positioned. 
The first step of the algorithm is to sample a value from an arbitrary proposal distribution.
Ideally, you want it to be be closer to the posterior distribution. For each iteration,
we sample a value from a proposal distribution, which here is a normal distribution 
centered on the current location. Then, we calculate the 
